Chern-Simons Modified General Relativity

Chern-Simons modified gravity is an effective extension of general relativity that captures leading-order, gravitational parity violation. Such an effective theory is motivated by anomaly cancelation in particle physics and string theory. In this review, we begin by providing a pedagogical derivation of the three distinct ways such an extension arises: (1) in particle physics, (2) from string theory and (3) geometrically. We then review many exact and approximate, vacuum solutions of the modified theory, and discuss possible matter couplings. Following this, we review the myriad astrophysical, solar system, gravitational wave and cosmological probes that bound Chern-Simons modified gravity, including discussions of cosmic baryon asymmetry and inflation. The review closes with a discussion of possible future directions in which to test and study gravitational parity violation.

==> Far-Field_v2.tex <==
In this section, we perform a PN expansion of the field equations and
obtain a solution in the form of a PN series. This solution then
allows us to read off the PPN parameters by comparing it to the
standard PPN super-metric [Eq.~(\ref{PPN})]. In this section we shall
follow closely the methods of~\cite{Will:1993ns}
and~\cite{Misner:1973cw} and indices shall be manipulated with the
Minkowski metric, unless otherwise specified.

Let us begin by expanding the field equations to second order in the
metric perturbation. Doing so we find that the Ricci and Cotton
tensors are given to second order by 
%
\ba
\label{Ricci-2nd-O}
R_{\mu \nu} &=& -\frac{1}{2} \left[\square_{\eta} h_{\mu \nu} - 2
  h_{\sigma(\mu,\nu)}{}^{\sigma} +  h_{,\mu \nu} \right] 
- \frac{1}{2} \left[ h^{\rho_\lambda} \left(2 h_{\rho(\mu,\nu)\lambda}
    - h_{\mu \nu,\rho\lambda} - h_{\rho\lambda,\mu \nu} \right) 
- \frac{1}{2} h^{\rho\lambda}{}_{,\mu} h_{\rho\lambda,\nu} +
h^{\lambda}{}_{\mu,\rho} h^{\rho}{}_{\nu,\lambda}  
\right. 
\\ \nonumber 
&-& \left. 
 h^{\rho}{}_{\mu,\lambda} h_{\rho\nu,}{}^{\lambda} 
+ \frac{1}{2} \left( h^{,\lambda}  - 2 h^{\lambda \rho}{}_{,\rho} \right)
\left( h_{\mu \nu,\lambda} - 2 h_{\lambda (\mu,\nu)} \right) \right] +
{\cal{O}}(h)^3, 
\nonumber \\
C_{\mu \nu} &=& - \frac{\dot{f}}{2} \tilde{\epsilon}^{0 \alpha
  \beta}{}_{(\mu} \left( \square_{\eta} h_{\nu) \beta,\alpha} -
  h_{\sigma \beta, \alpha \nu)}{}^{\sigma} \right) - \frac{\dot{f}}{2}
\tilde{\epsilon}^{0 \alpha \beta}{}_{(\mu} \left[ h \left(\square_{\eta}
      h_{\nu) \beta,\alpha} - h_{\sigma \beta, \alpha \nu)}{}^{\sigma}
    \right) + \frac{1}{2} \left( 2 h_{\nu) (\lambda,\alpha)} -
      h_{\lambda \alpha, \nu)} 
    \right) 
\right. 
\nonumber \\
&\times& \left.
\left( \square_{\eta}h^{\lambda}{}_{\beta} - 2
      h_{\sigma}{}^{(\lambda}{}_{,\beta)}{}^{\sigma} +
      h_{,\beta}{}^{\lambda} \right) - 2 \hat{Q}
    R_{\nu) \beta,\alpha} \right]  - \frac{\dot{f}}{4}
 \tilde{\epsilon}^{\sigma \alpha \beta}{}_{(\mu} \left( 2
   h^{0}{}_{(\sigma,\tau)} - h_{\sigma \tau,}{}^{0} \right) \left(
   h^{\tau}{}_{[\beta,\alpha] \nu)} -
   h_{\nu)[\beta,\alpha]}{}^{\tau} \right)
\nonumber \\
&-& \frac{\dot{f}}{2} h_{\mu \lambda} \tilde{\epsilon}^{0 \alpha \beta
  (\lambda} \left( \square_{\eta} h_{\nu) \beta,\alpha} - h_{\sigma
    \beta, \alpha \nu)}{}^{\sigma} \right)
- \frac{\dot{f}}{2} \tilde{\epsilon}^{0 \alpha \beta
  (\mu} \left( \square_{\eta} h^{\lambda)}{}_{\beta,\alpha} -
  h_{\sigma \beta, \alpha}{}^{\sigma \lambda)} \right) h_{\nu \lambda}
  + {\cal{O}}(h)^3.
\ea
%
where index contraction is carried out with the Minkowski metric and
where we have not assumed any gauge condition. The operator
$\hat{Q}(\cdot)$ takes the quadratic part of its operand [of
${\cal{O}}(h)^2$] and it is explained in more detail in
Appendix~\ref{derive-Cotton}, where the derivation of the expansion of
the Cotton tensor is presented in more detail. In this derivation, we
have used the definition of the Levi-Civita tensor
%
\ba
\epsilon_{\alpha \beta \gamma \delta} &=& (-g)^{1/2}
\tilde\epsilon_{\alpha\beta\gamma\delta} = \left(1 - \frac{1}{2} h
  \right) \tilde\epsilon_{\alpha\beta\gamma\delta} + {\cal{O}}(h)^2,
\\ \nonumber 
\epsilon^{\alpha \beta \gamma \delta} &=& -(-g)^{-1/2}
\tilde\epsilon^{\alpha\beta\gamma\delta} = -\left(1 + \frac{1}{2} h
  \right) \tilde\epsilon^{\alpha\beta\gamma\delta} + {\cal{O}}(h)^2.
\ea
%
Note that the PN expanded version of the linearized Ricci tensor of
Eq.~(\ref{Ricci-2nd-O}) agrees with previous
results~\cite{Will:1993ns}. Also note that if the Lorentz condition is
enforced, several terms in both expressions vanish identically and the
Cotton tensor to first order reduces to
Eq.~(\ref{linear-Lorentz-filed-eqs}), which agrees with previous
results~\cite{Jackiw:2003pm}.

Let us now specialize the analysis to the standard PPN gauge. For this
purpose, we shall impose the following gauge conditions
%
\ba
h_{jk,}{}^{k} - \frac{1}{2} h_{,j} &=& {\cal{O}}(4),
\nonumber \\
h_{0k,}{}^{k} - \frac{1}{2} h^{k}{}_{k,0} &=& {\cal{O}}(5),
\ea
%
where $h^{k}{}_{k}$ is the spatial trace of the metric perturbation.
Note that the first equation is the PN expansion of one of the Lorentz
gauge conditions, while the second equation is not.  This is the
reason why the previous equations where not expanded in the Lorentz
gauge.  Nonetheless, such a gauge condition does not uniquely fix the
coordinate system, since we can still perform an infinitesimal gauge
transformation that leaves the modified field equations invariant.
One can show that the Lorentz and PPN gauge are related to each other
by such a gauge transformation. In the PPN gauge, then, the Ricci
tensor takes the usual form
%
\ba
R_{00} &=& - \frac{1}{2} \nabla^2 h_{00} - \frac{1}{2} h_{00,i}
h_{00,}{}^{i} + \frac{1}{2} h^{ij} h_{00,ij} + {\cal{O}}(6),
\nonumber \\
R_{0i} &=& - \frac{1}{2} \nabla^2 h_{0i} - \frac{1}{4} h_{00,0i} + {\cal{O}}(5),
\nonumber \\
R_{ij} &=& - \frac{1}{2} \nabla^2 h_{ij} + {\cal{O}}(4),
\ea
%
which agrees with previous results~\cite{Will:1993ns}, while the
Cotton tensor reduces to
%
\ba
\label{expanded-Cotton}
C_{00} &=& {\cal{O}}(6),
\nonumber \\
C_{0i} &=& - \frac{1}{4} \dot{f} \tilde{\epsilon}^{0kl}{}_{i} \nabla^2
h_{0l,k} + {\cal{O}}(5), 
\nonumber \\
C_{ij} &=& - \frac{1}{2} \dot{f} \tilde{\epsilon}^{0kl}{}_{(i}
\nabla^2 h_{j) l,k} + {\cal{O}}(4),
\ea
%
where $\nabla = \eta^{ij} \partial_i \partial_j$ is the Laplacian of
flat space [see Appendix~\ref{derive-Cotton} for the derivation of
Eq.~(\ref{expanded-Cotton}).] Note again the explicit appearance of
two coupling terms of the Cotton tensor to the metric perturbation:
one to the transverse-traceless part of the spatial metric and the
other to the vector metric perturbation.  The PN expansions of the
linearized Ricci and Cotton tensor then allow us to solve the modified
field equations in the PPN framework.


==> PPN_v2.tex <==
\subsubsection{The ABC of PPN}
\label{abc}

In this section we summarize the basics of the PPN framework,
following~\cite{Will:1993ns}. This framework was first developed by
Eddington, Robertson and Schiff~\cite{Will:1993ns,Schiff:1960gi}, but
it came to maturity through the seminal papers of Nordtvedt and
Will~\cite{Nordtvedt:1968qs,1972ApJ...177..775N,1971ApJ...163..611W,1973ApJ...185...31W}.
In this section, we describe the latter formulation, since it is the
most widely used in experimental tests of gravitational theories.

The goal of the PPN formalism is to allow for comparisons of different
metric theories of gravity with each other and with experiment. Such
comparisons become manageable through a slow-motion, weak-field
expansion of the metric and the equations of motion, the so-called PN
expansion. When such an expansion is carried out to sufficiently high
but finite order, the resultant solution is an accurate approximation
to the exact solution in most of the spacetime.  This approximation,
however, does break down for systems that are not slowly-moving, such
as merging binary systems, or weakly gravitating, such as near the
apparent horizons of black hole binaries. Nonetheless, as far as solar
system tests are concerned, the PN expansion is not only valid but
also highly accurate.

The PPN framework employs an order counting-scheme that is similar to
that used in multiple-scale
analysis~\cite{Bender,Kevorkian,Yunes:2005nn,Yunes:2006iw}. The symbol
${\cal{O}}(A)$ stands for terms of order $\epsilon^A$, where $\epsilon
\ll 1$ is a PN expansion parameter. For convenience, it is customary
to associate this parameter with the orbital velocity of the system
$v/c = {\cal{O}}(1)$, which embodies the slow-motion approximation. By
the Virial theorem, this velocity is related to the Newtonian
potential $U$ via $U \sim v^2$, which then implies that $U =
{\cal{O}}(2)$ and embodies the weak-gravity approximation. These
expansions can be thought of as two independent series: one in inverse
powers of the speed of light $c$ and the other in positive powers of
Newton's gravitational constant.

Other quantities, such as matter densities and derivatives, can and
should also be classified within this order-counting scheme.  Matter
density $\rho$, pressure $p$ and specific energy density $\Pi$,
however, are slightly more complicated to classify because they are
not dimensionless.  Dimensionlessness can be obtained by comparing the
pressure and the energy density to the matter density, which we assume
is the largest component of the stress-energy tensor, namely $p/\rho
\sim \Pi/\rho = {\cal{O}}(2)$. Derivatives can also be classified in
this fashion, where we find that $\partial_t/\partial_x =
{\cal{O}}(1)$. Such a relation can be derived by noting that
$\partial_t \sim v^i \nabla_i$, which comes from the Euler equations
of hydrodynamics to Newtonian order.

With such an order-counting scheme developed, it is instructive to
study the action of a single neutral particle. The Lagrangian of this
system is given by
%
\ba
\label{L}
L &=& \left(g_{\mu \nu} u^{\mu} u^{\nu}\right)^{1/2},
\nonumber \\
&=& \left(-g_{00} - 2 g_{0i} v^i - g_{ij} v^i v^j\right)^{1/2}
\ea
%
where $u^{\mu} = dx^{\mu}/dt = (1,v^i)$ is the $4$-velocity of the
particle and $v^i$ is its $3$-velocity. From Eq.~(\ref{L}), note that
knowledge of $L$ to ${\cal{O}}(A)$ implies knowledge of $g_{00}$ to
${\cal{O}}(A)$, $g_{0i}$ to ${\cal{O}}(A-1)$ and $g_{ij}$ to
${\cal{O}}(A-2)$. Therefore, since the Lagrangian is already known to
${\cal{O}}(2)$ (the Newtonian solution), the first PN correction to
the equations of motion requires $g_{00}$ to ${\cal{O}}(4)$, $g_{0i}$
to ${\cal{O}}(3)$ and $g_{ij}$ to ${\cal{O}}(2)$. Such order counting
is the reason for calculating different sectors of the metric
perturbation to different PN orders.

A PPN analysis is usually performed in a particular background, which
defines a particular coordinate system, and in an specific gauge,
called the standard PPN gauge. The background is usually taken to be
Minkowski because for solar system experiments deviations due to
cosmological effects are negligible and can, in principle, be treated
as adiabatic corrections. Moreover, one usually chooses a standard PPN
frame, whose outer regions are at rest with respect to the rest frame
of the universe. Such a frame, for example, forces the spatial sector
of the metric to be diagonal and isotropic~\cite{Will:1993ns}. The
gauge employed is very similar to the PN expansion of the Lorentz
gauge of linearized gravitational wave theory. The differences between
the standard PPN and Lorentz gauge are of ${\cal{O}}(3)$ and they
allow for the presence of certain PPN potentials in the vectorial
sector of the metric perturbation.

The last ingredient in the PPN recipe is the choice of a stress-energy
tensor. The standard choice is that of a perfect fluid, given by
%
\be
T^{\mu \nu} = \left( \rho + \rho \Pi + p \right) u^{\mu} u^{\nu} + p
g^{\mu \nu}.
\ee
%
Such a stress-energy density suffices to obtain the PN expansion of
the gravitational field outside a fluid body, like the Sun, or of
compact binary system. One can show that the internal structure of the
fluid bodies can be neglected to 1~PN order by the effacement
principle~\cite{Blanchet:2002av} in GR. Such effacement principle
might actually not hold in modified field theories, but we shall study
this subject elsewhere~\cite{Alexander:2007:wip}.

With all these machinery, on can write down a
super-metric~\cite{Will:1993ns}, namely
%
\ba
\label{PPN}
g_{00} &=& - 1 + 2 U - 2 \beta U^2 - 2 \xi \Phi_W + \left( 2 \gamma
  + 2 + \alpha_3 + \zeta_1 
\right. 
\nonumber \\
&-& \left. 
 2 \xi\right) \Phi_1 + 2 \left(3 \gamma - 2 \beta + 1 + \zeta_2 + \xi
\right) \Phi_2 
\nonumber \\
&+& 2 \left(1 + \zeta_3 \right) \Phi_3 + 2 \left( 3 \gamma +  3
  \zeta_4 - 2 \xi \right) \Phi_4  - \left( \zeta_1 - 2 \xi \right)
  {\cal{A}}, 
\nonumber \\
g_{0i} &=& -\frac{1}{2} \left(4 \gamma + 3 + \alpha_1 - \alpha_2 +
  \zeta_1 - 2 \xi \right) V_i 
\nonumber \\
&-& \frac{1}{2} \left(1 + \alpha_2 -  \zeta_1 + 2 \xi \right) W_i,
\nonumber\\
g_{ij} &=& \left(1 + 2 \gamma U\right) \delta_{ij},
\ea
%
where $\delta_{ij}$ is the Kronecker delta and where the PPN
potentials ($U,\Phi_W,\Phi_1,\Phi_2,\Phi_3,\Phi_4,{\cal{A}},V_i,W_i$)
are defined in Appendix~\ref{def-PPN-Pot}. Equation~(\ref{PPN})
describes a super-metric theory of gravity, because it reduces to
different metric theories, such as GR or other alternative
theories~\cite{Will:1993ns}, through the appropriate choice of PPN
parameters
($\gamma,\beta,\xi,\alpha_1,\alpha_2,\alpha_3,\zeta_1,\zeta_2,\zeta_3,\zeta_4$).
One could obtain a more general form of the PPN metric by performing a
post-Galilean transformation on Eq.~(\ref{PPN}), but such a procedure
shall not be necessary in this paper.

The super-metric of Eq.~(\ref{PPN}) is parameterized in terms of a
specific number of PPN potentials, where one usually employs certain
criteria to narrow the space of possible potentials to consider.  Some
of these restriction include the following: the potentials tend to
zero as an inverse power of the distance to the source; the origin of
the coordinate system is chosen to coincide with the source, such that
the metric does not contain constant terms; and the metric
perturbations $h_{00}$, $h_{0i}$ and $h_{ij}$ transform as a scalar,
vector and tensor. The above restrictions are reasonable, but, in
general, an additional subjective condition is usually imposed that is
based purely on simplicity: the metric perturbations are not generated
by gradients or curls of velocity vectors or other generalized vector
functions. As of yet, no reason had arisen for relaxing such a
condition, but as we shall see in this paper, such terms are indeed
needed for CS modified theories.

What is the physical meaning of all these parameters? One can
understand what these parameters mean by calculating the generalized
geodesic equations of motion and conservation laws~\cite{Will:1993ns}.
For example, the parameter $\gamma$ measures how much space-curvature
is produced by a unit rest mass, while the parameter $\beta$
determines how much ``non-linearity'' is there in the superposition
law of gravity.  Similarly, the parameter $\xi$ determines whether
there are preferred-location effects, while $\alpha_i$ represent
preferred-frame effects. Finally, the parameters $\zeta_i$ measure the
amount of violation of conservation of total momentum. In terms of
conservation laws, one can interpret these parameters as measuring
whether a theory is fully conservative, with linear and angular
momentum conserved ($\zeta_i$ and $\alpha_i$ vanish),
semi-conservative, with linear momentum conserved ($\zeta_i$ and
$\alpha_3$ vanish), or non-conservative, where only the energy is
conserved through lowest Newtonian order. One can verify that in GR,
$\gamma = \beta = 1$ and all other parameters vanish, which implies
that there are no preferred-location or frame effects and that the
theory is fully conservative.

A PPN analysis of an alternative theory of gravity then reduces to
mapping its solutions to Eq.~(\ref{PPN}) and then determining the PPN
parameters in terms of intrinsic parameters of the theory. The
procedure is simply as follows: expand the modified field equations in
the metric perturbation and in the PN approximation; iteratively solve
for the metric perturbation to ${\cal{O}}(4)$ in $h_{00}$, to
${\cal{O}}(3)$ in $h_{0i}$ and to ${\cal{O}}(2)$ in $h_{ij}$; compare
the solution to the PPN metric of Eq.~(\ref{PPN}) and read off the PPN
parameters of the alternative theory. We shall employ this procedure
in Sec.~\ref{solutions} to obtain the PPN parameters of CS gravity.

\subsubsection{PPN Solution of CS gravity}
\label{solutions}

In this section we shall proceed to systematically solve the modified
field equation following the standard PPN iterative
procedure~\cite{Will:1993ns}.  We shall begin with the $00$ and $ij$
components of the metric to ${\cal{O}}(2)$, and then proceed with the
$0i$ components to ${\cal{O}}(3)$ and the $00$ component to
${\cal{O}}(4)$.  Once all these components have been solved for in
terms of PPN potentials, we shall be able to read off the PPN
parameters adequate to CS gravity.

%-----------------------------------------
\subsubsection{$h_{00}$ and $h_{ij}$ to ${\cal{O}}(2)$} 

Let us begin with the modified field equations for the scalar sector
of the metric perturbation. These equations are given to
${\cal{O}}(2)$ by
%
\be
\label{h00}
\nabla^2 h_{00} = -8 \pi \rho,  
\ee
%
because $T=-\rho$. Eq.~(\ref{h00}) is the Poisson equation, whose
solution in terms of PPN potentials is
%
\be
h_{00} = 2 U + {\cal{O}}(4). 
\ee
%

Let us now proceed with the solution to the field equation for the
spatial sector of the metric perturbation. This equation to
${\cal{O}}(2)$ is given by 
%
\be
\label{hij}
\nabla^2 h_{ij} +  \dot{f} \tilde{\epsilon}^{0kl}{}_{(i}
\nabla^2 h_{j) l,k} = -8 \pi \rho \delta_{ij},
\ee
%
where note that this is the first appearance of a Cotton tensor
contribution.  Since the Levi-Civita symbol is a constant and
$\dot{f}$ is only time-dependent, we can factor out the Laplacian and
rewrite this equation in terms of the effective metric
${\cal{H}}_{ij}$ as
%
\be
\label{effective-H}
\nabla^2 {\cal{H}}_{ij} = -8 \pi \rho \delta_{ij},
\ee
%
where, as defined in Sec.~\ref{CS},
%
\be
\label{effective-H-def}
{\cal{H}}_{ij} = h_{ij} + \dot{f} \tilde{\epsilon}^{0kl}{}_{(i} h_{j)
  l,k}.  
\ee
%
The solution of Eq.~(\ref{effective-H}) can be immediately found in
terms of PPN potentials as
%
\be
\label{effective-H-solved}
{\cal{H}}_{ij} = 2 U \delta_{ij} + {\cal{O}}(4),
\ee
%
which is nothing but Eq.~(\ref{formal-sol}). Recall, however, that in
Sec.~\ref{CS} we explicitly used the Lorentz gauge to simplify the
field equations, whereas here we are using the PPN gauge. The reason
why the solutions are the same is that the PPN and Lorentz gauge are
indistinguishable to this order.

Once the effective metric has been solved for, we can obtain the
actual metric perturbation following the procedure described in
Sec.~\ref{CS}. Combining Eq.~(\ref{effective-H-def}) with
Eq.~(\ref{effective-H-solved}), we arrive at the following
differential equation
%
\be
\label{hij-de}
h_{ij} + \dot{f} \tilde{\epsilon}^{0kl}{}_{(i} h_{j) l,k}
=  2 U \delta_{ij}. 
\ee
%
We look for solutions whose zeroth-order result is that predicted by
GR and the CS term is a perturbative correction, namely
%
\be
h_{ij} = 2 U \delta_{ij} + \dot{f} \zeta_{ij},
\ee
%
where $\zeta$ is assumed to be of ${\cal{O}}(\dot{f})^0$.  Inserting
this ansatz into Eq.~(\ref{hij-de}) we arrive at
%
\be
\zeta_{ij} +  \dot{f} \tilde{\epsilon}^{0kl}{}_{(i}
\zeta_{j) l,k} =  0,
\ee
%
where the contraction of the Levi-Civita symbol and the Kronecker
delta vanished. As in Sec.~\ref{CS}, note that the second term on the
left hand side is a second order correction and can thus be neglected
to discover that $\zeta_{ij}$ vanishes to this order.

The spatial metric perturbation to ${\cal{O}}(2)$ is then simply given
by the GR prediction without any CS correction, namely
%
\be
h_{ij} = 2 U \delta_{ij} + {\cal{O}}(4).
\ee
%
Physically, the reason why the spatial metric is unaffected by the CS
correction is related to the use of a perfect fluid stress-energy
tensor, which, together with the PPN gauge condition, forces the
metric to be spatially conformally flat. In fact, if the spatial
metric were not flat, then the spatial sector of the metric
perturbation would be corrected by the CS term.  Such would be the
case if we had pursued a solution to $2$ PN order, where the
Landau-Lifshitz pseudo-tensor sources a non-conformal correction to
the spatial metric~\cite{Blanchet:2002av}, or if we had searched for
gravitational wave solutions, whose stress-energy tensor
vanishes~\cite{Alexander:2004us,Alexander:2007:bgw}. In fact, one
can check that, in such a scenario, Eq.~(\ref{effective-H}) reduces to
that found
by~\cite{Jackiw:2003pm,Alexander:2004us,Alexander:2007:bgw,Alexander:2007:wip}
as $\rho \to 0$. We have then found that the weak-field expansion of
the gravitational field outside a fluid body, like the Sun or a
compact binary, is unaffected by the CS correction to ${\cal{O}}(2)$.


%-----------------------------------------
\subsubsection{$h_{0i}$ to ${\cal{O}}(3)$} 

Let us now look for solutions to the field equations for the vector
sector of the metric perturbation. The field equations to
${\cal{O}}(3)$ become
%
\ba
\label{h0i}
\nabla^2 h_{0i} + \frac{1}{2} h_{00,0i} + \frac{1}{2} \dot{f}
\tilde\epsilon^{0kl}{}_{i} \nabla^2h_{0l,k} 
= 16 \pi \rho v_i,
\ea
%
where we have used that $T^{0i} = -T_{0i}$. Using the lower order
solutions and the effective metric, as in Sec.~\ref{CS}, we obtain
%
\ba
\label{DE-h0i}
\nabla^2 {\cal{H}}_{0i} + U_{,0i} = 16 \pi \rho v_i,
\ea
%
where the vectorial sector of the effective metric is
%
\be
\label{H0i-vector}
{\cal{H}}_{0i} =  h_{0i} + \frac{1}{2} \dot{f}
\tilde\epsilon^{0kl}{}_{i} h_{0l,k}.
\ee
%
We recognize Eq.~(\ref{DE-h0i}) as the standard GR field equation to
${\cal{O}}(3)$, except that the dependent function is the effective
metric instead of the metric perturbation. We can thus solve this
equation in terms of PPN potentials to obtain
%
\be
\label{H0i-sol}
{\cal{H}}_{0i} = -\frac{7}{2} V_i - \frac{1}{2} W_i,
\ee
%
where we have used that the superpotential $X$ satisfies $X_{,0j} =
V_j - W_j$ (see Appendix~\ref{def-PPN-Pot} for the definitions.)
Combining Eq.~(\ref{H0i-vector}) with Eq.~(\ref{H0i-sol}) we arrive at
a differential equation for the metric perturbation, namely
%
\be
 h_{0i} + \frac{1}{2} \dot{f} \tilde\epsilon^{0kl}{}_{i} h_{0l,k} =
 -\frac{7}{2} V_i - \frac{1}{2} W_i.
\ee
%
Once more, let us look for solutions that are perturbation about the
GR prediction, namely
%
\be
h_{0i} =  -\frac{7}{2} V_i - \frac{1}{2} W_i + \dot{f} \zeta_i,
\ee
%
where we again assume that $\zeta_i$ is of
${\cal{O}}(\dot{f})^0$. The field equation becomes 
%
\be
\zeta_{i} + \frac{1}{2} \dot{f} \left(\nabla \times \zeta\right)_i
= \frac{1}{2} \left( \frac{7}{2} \left(\nabla \times V\right)_i
+ \frac{1}{2} \left(\nabla \times W \right)_i \right),
\ee
%
where $\left(\nabla \times A\right)^i = \epsilon^{ijk} \partial_j A_k$
is the standard curl operator of flat space. As in Sec.~\ref{CS}, note
once more that the second term on the left-hand side is again a second
order correction and we shall thus neglect it. Also note that the curl
of the $V_i$ potential happens to be equal to the curl of the $W_i$
potential. The solution for the vectorial sector of the actual
gravitational field then simplifies to
%
\be
h_{0i} =  -\frac{7}{2} V_i - \frac{1}{2} W_i + 2 \dot{f} \left(\nabla
  \times V\right)_i + {\cal{O}}(5).
\ee
%

We have arrived at the first contribution of CS modified gravity to
the metric for a perfect fluid source.  Chern-Simons gravity was
previously seen to couple to the transverse-traceless sector of the
metric perturbation for gravitational wave
solutions~\cite{Jackiw:2003pm,Alexander:2004us,Alexander:2007:bgw,Alexander:2007:wip}.
The CS correction is also believed to couple to Noether vector
currents, such as neutron currents, which partially fueled the idea
that this correction could be enhanced. However, to our knowledge,
this correction was never thought to couple to vector metric
perturbations. From the analysis presented here, we see that in fact
CS gravity does couple to such terms, even if the matter source is
neutrally charged. The only requirement for such couplings is that the
source is not static, {\emph{ie.}} that the object is either moving or
spinning relative to the PPN rest frame so that the PPN vector
potential does not vanish.  The latter is suppressed by a relative
${\cal{O}}(1)$ because in the far field the velocity of a compact
object produces a term of ${\cal{O}}(3)$ in $V_i$, while the spin
produces a term of ${\cal{O}}(4)$. In a later section, we shall
discuss some of the physical and observational implications of such a
modification to the metric.

%-----------------------------------------
\subsubsection{$h_{00}$ to ${\cal{O}}(4)$} 
A full analysis of the PPN structure of a modified theory of gravity
requires that we solve for the $00$ component of the metric
perturbation to ${\cal{O}}(4)$. The field equations to this order are 
%
\ba
\label{h00:2}
&-& \frac{1}{2} \nabla^2 h_{00} - \frac{1}{2} h_{00,i} h_{00,i} +
\frac{1}{2} h_{ij} h_{00,ij} = 4 \pi \rho \left[1 
\right. 
\nonumber \\
&+& \left. 
 2 \left( v^2 - U + \frac{1}{2} \Pi + \frac{3}{2} \frac{p}{\rho}
 \right)\right],
\ea
%
where the CS correction does not contribute at this order (see
Appendix~\ref{derive-Cotton}.)  Note that the $h_{0i}$ sector of the
metric perturbation to ${\cal{O}}(3)$ does not feed back into the
field equations at this order either. The terms that do come into play
are the $h_{00}$ and $h_{ij}$ sectors of the metric, which are not
modified to lowest order by the CS correction. The field equation,
thus, reduce to the standard one of GR, whose solution in terms of PPN
potentials is
%
\be
h_{00} = 2 U - 2 U^2 + 4 \Phi_1 + 4 \Phi_2 + 2 \Phi_3 + 6 \Phi_4 +
{\cal{O}}(6). 
\ee
%
We have thus solved for all components of the metric perturbation to 1
PN order beyond the Newtonian answer, namely $g_{00}$ to
${\cal{O}}(4)$, $g_{0i}$ to ${\cal{O}}(3)$ and $g_{ij}$ to
${\cal{O}}(2)$.

%-----------------------------------------
\subsubsection{PPN Parameters for CS  Gravity}
We now have all the necessary ingredients to read off the PPN
parameters of CS modified gravity. Let us begin by writing the full
metric with the solutions found in the previous subsections:
%
\ba
\label{CS-full-metric}
g_{00} &=& -1 + 2 U - 2 U^2 + 4 \Phi_1 + 4 \Phi_2 + 2 \Phi_3 + 6 \Phi_4 +
{\cal{O}}(6), 
\nonumber \\
g_{0i} &=& -\frac{7}{2} V_i - \frac{1}{2} W_i + 2 \dot{f} \left(\nabla
  \times V\right)_i + {\cal{O}}(5),
\nonumber \\
g_{ij} &=& \left(1 + 2 U \right) \delta_{ij} + {\cal{O}}(4). 
\ea
%
One can verify that this metric is indeed a solution of
Eqs.~(\ref{h00}), (\ref{hij}), (\ref{h0i}) and~(\ref{h00:2}) to the
appropriate PN order and to first order in the CS coupling parameter.
Also note that the solution of Eq.~(\ref{CS-full-metric})
automatically satisfies the constraint $^{\star}R R = 0$ to linear
order because the contraction of the Levi-Civita symbol with two
partial derivatives vanishes. Such a solution is then allowed in CS
gravity, just as other classical solutions are~\cite{Guarrera:2007tu},
and the equations of motion for the fluid can be obtained directly
from the covariant derivative of the stress-energy tensor.

We can now read off the PPN parameters of the CS modified theory by
comparing Eq.~(\ref{PPN}) to Eq.~(\ref{CS-full-metric}). A visual
inspection reveals that the CS solution is identical to the classical
GR one, which implies that $\gamma = \beta = 1$, $\zeta = 0$ and
$\alpha_1 = \alpha_2 = \alpha_3 = \xi_1 = \xi_2 = \xi_3 = \xi_4 = 0$
and there are no preferred frame effects. However, Eq.~(\ref{PPN})
contains an extra term that cannot be modeled by the standard PPN
metric of Eq.~(\ref{PPN}), namely the curl contribution to $g_{0i}$.
We then see that the PPN metric must be enhanced by the addition of a
curl-type term to the $0i$ components of the metric, namely
%
\ba
g_{0i} &\equiv& -\frac{1}{2} \left(4 \gamma + 3 + \alpha_1 - \alpha_2 +
  \zeta_1 - 2 \xi \right) V_i 
\nonumber \\
&-& \frac{1}{2} \left(1 + \alpha_2 -  \zeta_1 + 2 \xi \right) W_i +
\chi \left(r \nabla \times V\right)_{i},
\ea
%
where $\chi$ is a {\emph{new}} PPN parameter and where we have
multiplied the curl operator by the radial distance to the source,
$r$, in order to make $\chi$ a proper dimensionless parameter. Note
that there is no need to introduce any additional PPN parameters
because the curl of $W_i$ equals the curl of $V_i$. In fact, we could
have equally parameterized the new contribution to the PPN metric in
terms of the curl of $W_i$, but we chose not to because $V_i$ appears
more frequently in PN theory. For the case of CS modified gravity,
the new $\chi$ parameter is simply
%
\be
\chi = 2 \frac{\dot{f}}{r}, 
\ee
%
which is dimensionless since $\dot{f}$ has units of length. If an
experiment could measure or place bounds on the value of $\chi$, then
$\dot{f}$ could also be bounded, thus placing a constraint on the CS
coupling parameter.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Astrophysical Implications}
\label{consequences}

In this section we shall propose a physical interpretation to the CS
modification to the PPN metric and we shall calculate some GR
predictions that are modified by this correction. This section,
however, is by no means a complete study of all the possible
consequences of the CS correction, which is beyond the scope of this
paper.

Let us begin by considering a system of $A$ nearly spherical bodies,
for which the gravitational vector potentials are
simply~\cite{Will:1993ns}
%
\ba
\label{vector-pot}
V^i &=& \sum_A \frac{m_A}{r_A} v^i_A + \frac{1}{2} \sum_A
\left(\frac{J_A}{r_A^2} \times n_A\right)^i,
\\ \nonumber 
W^i &=& \sum_A \frac{m_A}{r_A} \left(v_A \cdot n_A\right) n_A^i +
\frac{1}{2} \sum_A \left(\frac{J_A}{r_A^2} \times n_A\right)^i,
\ea
%
where $m_A$ is the mass of the $A$th body, $r_A$ is the field point
distance to the $A$th body, $n_A^i = x^i_A/r_A$ is a unit vector
pointing to the $A$th body, $v_A$ is the velocity of the $A$th body
and $J_A^i$ is the spin-angular momentum of the $A$th body. For
example, the spin angular momentum for a Kerr spacetime is given by
$J^i = m^2 a^i$, where $a$ is the dimensionless Kerr spin parameter.
Note that if $A = 2$ then the system being modeled could be a binary
of spinning compact objects, while if $A=1$ it could represent the
field of the sun or that of a rapidly spinning neutron star or pulsar.

In obtaining Eq.~(\ref{vector-pot}), we have implicitly assumed a
point-particle approximation, which in classical GR is justified by
the effacement principle. This principle postulates that the internal
structure of bodies contributes to the solution of the field equations
to higher PN order. One can verify that this is indeed the case in
classical GR, where internal structure contributions appear at $5$ PN
order. In CS gravity, however, it is a priori unclear whether an
analogous effacement principle holds because the CS term is expected
to couple with matter current via standard model-like interactions. If
such is the case, it is possible that a ``mountain'' on the surface of
a neutron star~\cite{Owen:2005fn} or an r-mode
instability~\cite{Chandrasekhar:1992pr,Friedman:1978hf,Lindblom:1998wf}
enhances the CS contribution. In this paper, however, we shall neglect
these interactions, and relegate such possibilities to future
work~\cite{Alexander:2007:wip}.

With such a vector potential, we can calculate the CS correction to
the metric. For this purpose, we define the correction $\delta g_{0i}
\equiv g_{0i} - g_{0i}^{(GR)}$, where $g_{0i}^{(GR)}$ is the GR
prediction without CS gravity. We then find that the CS corrections is
given by 
%
\be
\label{CS-term}
\delta g_{0i} = 2  \sum_A \frac{\dot{f}}{r_A} \left[ \frac{m_A}{r_A}
  \left(v_A \times n_A \right)^i - \frac{J^i_A}{2 r_A^2} + \frac{3}{2}
  \frac{\left(J_A \cdot n_A\right)}{r_A^2} n_A^i \right],
\ee
%
where the $\cdot$ operator is the flat-space inner product and where
we have used the identities $\tilde\epsilon_{ijk} \tilde\epsilon_{klm}
= \delta_{il} \delta_{jm} - \delta_{im} \delta_{jl}$ and
$\tilde\epsilon_{ilk} \tilde\epsilon_{jlm} = 2 \delta_{ij}$.  Note
that the first term of Eq.~(\ref{CS-term}) is of ${\cal{O}}(3)$, while
the second and third terms are of ${\cal{O}}(4)$ as previously
anticipated. Also note that $\dot{f}$ couples both to the spin and
orbital angular momentum. Therefore, whether the system under
consideration is the Solar system ($v^i$ of the Sun is zero while
$J^i$ is small), the Crab pulsar ($v^i$ is again zero but $J^i$ is
large) or a binary system of compact objects (neither $v^i$ nor $J^i$
vanish), there will in general be a non-vanishing coupling between the
CS correction and the vector potential of the system.

From the above analysis, it is also clear that the CS correction
increases with the non-linearity of the spacetime. In other words, the
CS term is larger not only for systems with large velocities and
spins, but also in regions near the source. For a binary system, this
fact implies that the CS correction is naturally enhanced in the last
stages of inspiral and during merger. Note that this enhancement is
{\emph{different}} from all previous enhancements proposed, since it
does not require the presence of
charge~\cite{Alexander:2007:wip,Alexander:2007:bgw}, a fifth dimension
with warped
compactifications~\cite{randall:1999:lmh,randall:1999:atc}, or a
vanishing string
coupling~\cite{Brandenberger:1988:sit,Tseytlin:1991xk,Nayeri:2005ck,Sun:2006sd,Wesley:2005bd,Alexander:2000:bgi,Brandenberger:2001:lpi,Battefeld:2005av,Brandenberger:2006vv,Brandenberger:2007zz,Brax:2004xh}.
Unfortunately, the end of the inspiral stage coincides with the edge
of the PN region of validity and, thus, a complete analysis of such a
natural enhancement will have to be carried out through numerical
simulations.

In the presence of a source with the vector potentials of
Eq.~(\ref{vector-pot}), we can write the vectorial sector of the
metric perturbation in a suggestive way, namely
%
\ba
\label{effective}
g_{0i} &=& \sum_A - \frac{7}{2} \frac{m_A}{r_A} v^i_A 
- \sum_A \frac{m_A}{6 r_A^2} \left(v_A - v_A^{(eff)}\right)^i
\\ \nonumber 
&-& \frac{1}{2} \sum_A n_A^i \frac{m_A}{r_A} v^{(eff)}_A \cdot n_A  
- 2 \sum_A \left[ \frac{J_A^{(eff)}}{r_A^2} \times n_A \right]^i,
\ea
%
where we have defined an effective velocity and angular momentum
vector via
%
\ba
v_{A(eff)}^i &=& v^i_A - 6 \dot{f} \frac{J^i_A}{m_A r_A^2},
\nonumber \\
J_{A(eff)}^i &=& J^i_A - \dot{f} m_A v_A^i,
\ea
%
or in terms of the Newtonian orbital angular momentum $L^i_{A (N)} =
r_A \times p_A$ and linear momentum $p^i_{A (N)} = m_A v_A^i$
%
\ba
L^i_{A(eff)} &=& L^i_{A(N)} - 6 \dot{f} \left(n_A \times J_A\right)^i,
\nonumber \\
J^i_{A(eff)} &=& J_A^i - \dot{f} p_A^i.
\ea
%
From this analysis, it is clear that the CS corrections seems to
couple to both a quantity that resembles the orbital and the spin
angular momentum vector. Note that when the spin angular momentum
vanishes the vectorial metric perturbation is identical to that of a
spinning moving fluid, but where the spin is induced by the coupling
of the orbital angular momentum to the CS term. 

The presence of an effective CS spin angular momentum in non-spinning
sources leads to an interesting physical interpretation.  Let us model
the field that sources $\dot{f}$ as a fluid that permeates all of
spacetime. This field could be, for example, a model-independent
axion, inspired by the quantity introduced in the standard model to
resolve the strong CP problem~\cite{Dine:1981rt}. In this scenario,
then the fluid is naturally ``dragged'' by the motion of any source
and the CS modification to the metric is nothing but such dragging.
This analogy is inspired by the ergosphere of the Kerr solution, where
inertial frames are dragged with the rotation of the black hole. In
fact, one could push this analogy further and try to construct the
shear and bulk viscosity of such a fluid, but we shall not attempt
this here. Of course, this interpretation is to be understood only
qualitatively, since its purpose is only to allow the reader to
picture the CS modification to the metric in physical terms.

An alternative interpretation can be given to the CS modification in
terms of the gravito-electro-magnetic (GED)
analogy~\cite{1986bhmp.book.....T,Mashhoon:2003ax}, which shall allow
us to easily construct the predictions of the modified theory. In this
analogy, one realizes that the PN solution to the linearized field
equations can be written in terms of a potential and vector potential,
namely
%
\be
ds^2 = - \left(1 - 2 \Phi \right) dt^2 - 4 \left(A \cdot dx \right) dt +
\left(1 + 2 \Phi \right) \delta_{ij} dx^i dx^j,
\ee
%
where $\Phi$ reduces to the Newtonian potential $U$ in the Newtonian
limit~\cite{Mashhoon:2003ax} and $A^i$ is a vector potential related
to the metric via $A_i = -g_{0i}/4$. One can then construct GED fields
in analogy to Maxwell's electromagnetic theory via
%
\ba
E^i &=& - \left(\nabla\Phi\right)^i - \partial_t \left(\frac{1}{2} A^i \right), 
\nonumber \\
B^i &=& \left(\nabla \times A\right)^i,
\ea
%
which in terms of the vectorial sector of the metric perturbation
becomes
%
\ba
E^i &=& - \left(\nabla\Phi\right)^i + \frac{1}{8} \dot{g}^i,
\nonumber \\
B^i &=& -\frac{1}{4} \left(\nabla \times g\right)^i,
\ea
%
where we have defined the vector $g^i = g_{0i}$. The geodesic
equations for a test particle then reduce to the Lorentz force law,
namely
%
\ba
F^i = - m E^i  - 2 m \left(v \times B\right)^i.
\ea
%

We can now work out the effect of the CS correction on the GED fields
and equations of motion. First note that the CS correction only
affects $g$. We can then write the CS modification to the Lorentz
force law by defining $\delta a^i = a^i - a^i_{(GR)}$, where
$a^i_{(GR)}$ is the acceleration vector predicted by GR, to obtain,
%
\be
\delta a^i = \frac{1}{8} \delta\dot{g}^i + \frac{1}{2} \left(v
  \times \delta\Omega\right)^i,
\ee
%
where we have defined the angular velocity
%
\be
\delta \Omega^i = \left(\nabla \times \delta g\right)^i.
\ee
%
The time derivative of the vector $g^i$ is of ${\cal{O}}(5)$ and can
thus be neglected, but the angular velocity cannot and it is given by
%
\be
\label{ang-vel}
\delta\Omega^i = - \sum_A \dot{f} \frac{m_A}{r_A^3} \left[ 3 \left(v_A \cdot
    n_A\right) n_A^i - v_A^i \right],
\ee
%
which is clearly of ${\cal{O}}(3)$. Note that although the first term
between square brackets cancels for circular orbits because $n_A^i$ is
perpendicular to $v_A^i$ to Newtonian order, the second term does not.
The angular velocity adds a correction to the acceleration of
${\cal{O}}(4)$, namely
%
\be
\label{acc}
\delta a^i = -\frac{3}{2} \sum_A \dot{f} \frac{m_A}{r_A^3} \left(v_A
  \cdot n_A \right) \left(v_A \times n_A\right)^i,
\ee
%
which for a system in circular orbit vanishes to Newtonian order. One
could use this formalism to find the perturbations in the motion of
moving objects by integrating Eq.~(\ref{acc}) twice.  However, for
systems in a circular orbit, such as the Earth-Moon system or compact
binaries, this correction vanishes to leading order. Therefore, lunar
ranging experiments~\cite{Murphy:2007nt} might not be able to
constraint $\dot{f}$.

Another correction to the predictions of GR is that of the precession
of gyroscopes by the so-called Lense-Thirring or frame-dragging
effect. In this process, the spin angular momentum of a source twists
spacetime in such a way that gyroscopes are dragged with it. The
precession angular velocity depends on the vector sector of the metric
perturbation via Eq.~(\ref{ang-vel}). Thus, the full Lense-Thirring
term in the precession angular velocity of precessing gyroscopes is
%
\be 
\Omega^i_{LT} = - \frac{1}{r_A^3} \sum_A J_{A(eff)}^i - 3 n^i_A
\left(J_{A(eff)} \cdot n_A \right)^i.  
\ee
%
Note that this angular velocity is identical to the GR prediction,
except for the replacement $J_A^i \to J^i_{A(eff)}$. In CS modified
gravity, then, the Lense-Thirring effect is not only produced by the
spin angular momentum of the gyroscope but also by the orbital angular
momentum that couples to the CS correction. Therefore, if an
experiment were to measure the precession of gyroscopes by the
curvature of spacetime (see, for example, Gravity Probe
B~\cite{GravityProbeB}) one could constraint $\dot{f}$ and thus some
intrinsic parameters of string theory. Note, however, that the CS
correction depends on the velocity of the bodies with respect to the
inertial PPN rest-frame. In order to relate these predictions to the
quantities that are actually measured in the experiment, one would
have to transform to the experiment's frame, or perhaps to a basis
aligned with the direction of distant stars~\cite{Will:1993ns}.

Are there other experiments that could be performed to measure such a
deviation from GR? Any experiment that samples the vectorial sector of
the metric would in effect be measuring such a deviation.  In this
paper, we have only discussed modifications to the frame-dragging
effect and the acceleration of bodies through the GED analogy, but
this need not be the only corrections to classical GR predictions. In
fact, any predictions that depends on $g_{0i}$ indirectly, for example
via Christoffel symbols, will probably also be modified unless the
corrections is fortuitously canceled. In this paper, we have laid the
theoretical foundations of the weak-field correction to the metric due
to CS gravity and studied some possible corrections to classical
predictions. A detailed study of other corrections is beyond the scope
of this paper.


==> conclusion_v1.tex <==
Chern-Simons modified gravity is a well-defined theory that models parity violation in the gravitational interaction. We have here reviewed the basic equations of this theory and discussed its motivation from particle physics and string theory. We have then summarized studies of exact and approximate solutions, which have led to calculations of parity-violating gravitational observables. We have also reviewed how such observables are still being searched for with astrophysical experiments and cosmological observations, which have already led to interesting constraints on the theory. 

The modified theory can be classified into a non-dynamical or a dynamical model. We have explained that in the former the CS scalar field is treated as an {\emph{a priori}} prescribed, external field, while in the latter this field is obtained by consistently solving its evolution equation and the modified field equations. The non-dynamical model has been found to be rather contrived and sometimes even over-constrained, when studying perturbations and exact solutions for non-rotating black holes, mainly due to additional differential conditions that it requires. The dynamical model is only now beginning to be studied in depth and so far it has led to no fundamental theoretical problems.   

Much work, however, remains to be done in order to fully understand the effects of parity violation in the dynamical formulation of CS modified gravity. Of particular importance is the CS modification to gravitational waves generated by binary black hole or neutron star mergers, since these are primary sources for gravitational wave detectors. During such violent events, the strong curvature of the background should enhance the CS correction, possibly leading to observable corrections in the gravitational wave spectrum. 

Another interesting prospect is that of the coupling of fermions to the CS correction. Certain astrophysical processes, such as gamma-ray bursts, involve large fermion currents, as well as strong gravitational fields, both of which will in principle enhance the CS correction. A full magnetohydrodynamic treatment of these events in CS modified gravity could also lead to interesting electromagnetic signatures of gravitational parity violation. 

Regardless of the astrophysical scenario, or of the expected magnitude of the CS correction, the search for parity breaking is a fundamental effort in our attempts to understand the cosmos. Only through the study of parity violation in gravitational interactions can we identify its signatures in observations and experiments. In turn, such signatures, or lack thereof, would provide interesting hints toward the unification of the gravitational and quantum interaction. Such an interplay between theory and experiment has always been and remains at the heart of physics, and only through it shall we be able to truly understand the secrets of our Universe.    

